Neural-Augmented Static Analysis of Android Communication

We address the problem of discovering communication links between applications in the popular Android mobile operating system, an important problem for security and privacy in Android. Any scalable static analysis in this complex setting is bound to produce an excessive amount of false-positives, rendering it impractical. To improve precision, we propose to augment static analysis with a trained neural-network model that estimates the probability that a communication link truly exists. We describe a neural-network architecture that encodes abstractions of communicating objects in two applications and estimates the probability with which a link indeed exists. At the heart of our architecture are type-directed encoders (TDE), a general framework for elegantly constructing encoders of a compound data type by recursively composing encoders for its constituent types. We evaluate our approach on a large corpus of Android applications, and demonstrate that it achieves very high accuracy. Further, we conduct thorough interpretability studies to understand the internals of the learned neural networks.

==> implementation.tex <==
\section{Implementation}
The design decisions and choices of hyperparameters are summarized
in Table \ref{tab:hyperparameters}.
Note that the very last activation of sigmoid
ensures that the output of our model is within $[0,1]$, denoting
the probability our model thinks the link being true.
\begin{table}
  \centering
  \begin{tabular}{lll}
    \toprule
     \multicolumn{2}{c}{Hyperparameter} &  \multicolumn{1}{c}{Choice} \\
    \midrule
    Embedding layer & dimension & 16 \\
    \midrule
    \multirow{4}{*}{Vary-sized CNN} & kernel sizes & [1, 3, 5, 7] \\
    & kernel counts & [8, 16, 32, 64] \\
    & activation & relu \\
    & pooling & max \\
    \midrule
    \multicolumn{2}{l}{Summarizing function} & sum \\
    \midrule
    \multirow{2}{*}{Single layer perceptron} & dimensions & 64 \\
    & activation & relu \\
    \midrule
    \multirow{2}{*}{Multilayer perceptron} & dimensions & [64, 1] \\
    & activation & [relu, $\sigma$] \\
    %% \multirow{8}{*}{Encoder}
    %Encoder
    %& Base encoder
    %  & Char encoder
    %    & Embedding layer
    %      & dimension & 16 \\
    %% & \multirow{7}{*}{Constructor}
    %& Constructor
    %  % & \multirow{4}{*}{{List}
    %  & List
    %    % & \multirow{4}{*}{Vary-sized CNN}
    %    & Vary-sized CNN
    %      & kernel sizes & [1, 3, 5, 7] \\
    %& & & & kernel counts & [8, 16, 32, 64] \\
    %& & & & activation & $\relu$ \\
    %& & & & pooling & $\max$ \\
    %& & Set
    %    & & summarizing function & sum \\
    %% & & \multirow{2}{*}{Product}
    %& & Product
    %    % & \multirow{2}{*}{Single layer perceptron}
    %    & Single layer perceptron
    %      & dimension & 64 \\
    %& & & & activation & $\relu$ \\
    %% \multirow{2}{*}{Classifier}
    %Classifier
    %% & & & \multirow{2}{*}{Multilayer perceptron}
    %& & & Multilayer perceptron
    %      & dimensions & [16, 1] \\
    %& & & & activations & [$\relu$, $\sigmoid$] \\
    \bottomrule
  \end{tabular}
  \caption{\linn instantiation and choices of  hyperparameters}
  \label{tab:hyperparameters}
\end{table}

We choose \emph{cross entropy loss} as the loss function for our binary classification task.
Given two distribution $p, q$ over finite set $Y$,
\emph{cross entropy} measures the difference between two probability distributions
by $- \sum_{y \in Y} p(y) \log q(y)$.
Specifically, for our binary classification, it becomes
\begin{align}
  cross\_entropy(y, \hat{p})
  = \begin{cases}
    \log \hat{p} & \text{for } y = 1, \\
    \log (1 - \hat{p}) & \text{for } y = 0,
  \end{cases}
\end{align}
for truth $y \in \cpara{0, 1}$ (link or no),
and output $\hat{p} \in [0, 1]$ (likelihood of a link).
Note that in this case, we have $Y = \cpara{0, 1}$,
true distribution $p(y) = 1$ and $p(1-y) = 0$ for truth $y$,
and predicted distribution $q(1)=\hat{p}$ and $q(1)=1 - \hat{p}$ for output $\hat{p}$.
Our loss function thus becomes,
\begin{align}
  l(h, \tuple{y, (\abs{\intent}, \abs{\filter})}) = cross\_entropy(y, h(\abs{\intent}, \abs{\filter})),
\end{align}
for model $h$ and training instance $\tuple{y, (\abs{\intent}, \abs{\filter})}$.

% \paragraph{Optimization}
% The training then is the process of minimizing the loss
% with respect to the training parameters
% \begin{align}
%   \minimize_{\theta} L_{D, \theta}
% \end{align}
% using \emph{gradient descent}.
% The idea is to start with a random set of parameters $\theta^{(0)}$
% and iteratively update it using the gradient with the current parameterization
% \begin{align}
%   \theta^{(i+1)} = \theta^{(i)} - \eta \frac{\partial L}{\partial \theta}
% \end{align}
% with learning rate $\eta$,
% until we reached certain number of iterations,
% the parameters is good enough,
% the progress is too slow,
% or etc.
% Practically, one often use \emph{stochastic gradient descent (SGD)},
% where the gradient $\frac{\partial l_{x}}{\partial \theta}$ is computed
% over a randomly sampled training instance $x$
% rather than the entire training set.
% This involves much less computation and thus faster training.


We implemented the above \linn with the above hyperparameters and loss function
in Python using Keras with Tensorflow backend.\footnote{The code can be found
online at \note{<github repo url>}.}
We use RMSprop \cite{tieleman2012lecture}, a variation of stochastic gradient descent (SGD)
with momentum and adaptive learning rate,
as the optimizer for the objective function.

